Residual Stream Analysis with Multi-Layer SAEs

Sparse autoencoders (SAEs) are a promising approach to interpreting the internal representations of transformer language models. However, SAEs are usually trained separately on each transformer layer, making it difficult to use them to study how information flows across layers. To solve this problem, we introduce the multi-layer SAE (MLSAE): a single SAE trained on the residual stream activation vectors from every transformer layer. Given that the residual stream is understood to preserve information across layers, we expected MLSAE latents to 'switch on' at a token position and remain active at later layers. Interestingly, we find that individual latents are often active at a single layer for a given token or prompt, but the layer at which an individual latent is active may differ for different tokens or prompts. We quantify these phenomena by defining a distribution over layers and considering its variance. We find that the variance of the distributions of latent activations over layers is about two orders of magnitude greater when aggregating over tokens compared with a single token. For larger underlying models, the degree to which latents are active at multiple layers increases, which is consistent with the fact that the residual stream activation vectors at adjacent layers become more similar. Finally, we relax the assumption that the residual stream basis is the same at every layer by applying pre-trained tuned-lens transformations, but our findings remain qualitatively similar. Our results represent a new approach to understanding how representations change as they flow through transformers. We release our code to train and analyze MLSAEs at https://github.com/tim-lawson/mlsae.

==> entropy/figure.tex <==
\newcommand{\addplotentropy}[2]{
	\addplot+ [mark=*] table [
			col sep=comma,
			x=#1,
			y=rel,
		]{#2}
}
\newcommand{\addplotentropyx}[1]{
	\addplotentropy{expansion_factor}{#1}
}
\newcommand{\addplotentropyk}[1]{
	\addplotentropy{k}{#1}
}
\begin{tikzpicture}
	\begin{groupplot}[
			scale only axis,
			width=2in,
			height=2in,
			group style={
					group size=2 by 1,
					horizontal sep=0.125in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			cycle list/Paired,
			title style={
					anchor=north,
					at={(0.5,1.1)},
					font=\small
				},
			y label style={
					anchor=south,
					at={(-0.2,.5)},
					font=\large,
				},
			ymin=0.45,
			ymax=0.875,
			xmode=log,
			grid=major,
			legend cell align={left},
			legend columns=2,
			legend style={
					anchor=south,
					at={(0,-0.75)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\nextgroupplot[
			title={Sparsity $k=32$},
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={\Large $\frac{\text{Mean Entropy}}{\ln n_L}$},
			xmin=0.5,
			xmax=512,
		]
		\addplotentropyx{entropy/pythia-70m-deduped/expansion_factor.csv};
		\addplotentropyx{entropy/pythia-70m-deduped-lens/expansion_factor.csv};
		\addplotentropyx{entropy/pythia-160m-deduped/expansion_factor.csv};
		\addplotentropyx{entropy/pythia-160m-deduped-lens.csv};
		\addplotentropyx{entropy/pythia-410m-deduped.csv};
		\addplotentropyx{entropy/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotentropyx{entropy/pythia-1b-deduped.csv};
		\addplotentropyx{entropy/pythia-1.4b-deduped.csv};
		\addplotentropyx{entropy/gemma2b.csv};
		\addplotentropyx{entropy/llama3b.csv};
		\addplotentropyx{entropy/gpt2.csv};
		\draw[dashed,gray] (axis cs:64,1e-1) -- (axis cs:64,1);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
		]
		\addplotentropyk{entropy/pythia-70m-deduped/sparsity_k.csv};
		\addplotentropyk{entropy/pythia-70m-deduped-lens/sparsity_k.csv};
		\addplotentropyk{entropy/pythia-160m-deduped/sparsity_k.csv};
		\addplotentropyk{entropy/pythia-160m-deduped-lens.csv};
		\addplotentropyk{entropy/pythia-410m-deduped.csv};
		\addplotentropyk{entropy/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotentropyk{entropy/pythia-1b-deduped.csv};
		\addplotentropyk{entropy/pythia-1.4b-deduped.csv};
		\addplotentropyk{entropy/gemma2b.csv};
		\addplotentropyk{entropy/llama3b.csv};
		\addplotentropyk{entropy/gpt2.csv};
		\draw[dashed,gray] (axis cs:32,1e-1) -- (axis cs:32,1);
		\addlegendentry{Pythia-70m}
		\addlegendentry{Pythia-70m with tuned lens}
		\addlegendentry{Pythia-160m}
		\addlegendentry{Pythia-160m with tuned lens}
		\addlegendentry{Pythia-410m}
		\addlegendentry{Pythia-410m with tuned lens}
		\addlegendentry{Pythia-1b}
		\addlegendentry{Pythia-1.4b}
		\addlegendentry{Gemma 2 2B}
		\addlegendentry{Llama 3.2 3B}
		\addlegendentry{GPT-2 small}
	\end{groupplot}
\end{tikzpicture}


==> entropy/model_name/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			scale only axis,
			width=4.5in,
			height=1.5in,
			group style={
					group size=1 by 2,
					vertical sep=0.75in,
				},
			xbar,
			xticklabel style={/pgf/number format/fixed},
			y dir=reverse,
			enlarge y limits=true,
			symbolic y coords={
					Pythia-70m,
					Pythia-160m,
					Pythia-410m,
					Pythia-1b,
					Pythia-1.4b,
					gemma-2-2b,
					Llama-3.2-3B,
					gpt2
				},
			ytick=data,
			yticklabels={
					Pythia-70m,
					Pythia-160m,
					Pythia-410m,
					Pythia-1b,
					Pythia-1.4b,
					Gemma 2 2B,
					Llama 3.2 3B,
					GPT-2 small
				},
			xtick align=outside,
			ytick align=outside,
			tick pos=left,
			axis x line*=left,
			axis y line*=left,
			axis line style=semithick,
			every tick/.style={black,semithick},
			legend cell align={left},
			legend columns=1,
			legend style={
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\nextgroupplot[
			xlabel={Mean Entropy / $\ln n_L$},
			xmin=0,
			xmax=1,
			bar width=0.0375in,
			legend pos=north east,
		]
		\addplot+ [Paired-A] table [
				col sep=comma,
				y=model_name,
				x=rel,
			]{entropy/model_name/without_tuned_lens.csv};
		\addplot+ [Paired-B] table [
				col sep=comma,
				y=model_name,
				x=rel,
			]{entropy/model_name/with_tuned_lens.csv};
		\addlegendentry{Standard}
		\addlegendentry{Tuned lens}
	\end{groupplot}
\end{tikzpicture}

==> heatmaps/with_tuned_lens/model_name/aggregate/counts/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 3,
					vertical sep=0.25in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Pythia-70m with tuned lens},
			ytick={0.5,1.5,...,5.5},
			yticklabels={$0$,,,,,$5$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/model_name/aggregate/counts/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m with tuned lens},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/with_tuned_lens/model_name/aggregate/counts/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m with tuned lens},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/with_tuned_lens/model_name/aggregate/counts/pythia-410m-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/with_tuned_lens/model_name/aggregate/probs/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 3,
					vertical sep=0.25in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Pythia-70m with tuned lens},
			ytick={0.5,1.5,...,5.5},
			yticklabels={$0$,,,,,$5$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/model_name/aggregate/probs/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m with tuned lens},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/with_tuned_lens/model_name/aggregate/probs/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m with tuned lens},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/with_tuned_lens/model_name/aggregate/probs/pythia-410m-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/with_tuned_lens/model_name/aggregate/totals/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 3,
					vertical sep=0.25in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Pythia-70m with tuned lens},
			ytick={0.5,1.5,...,5.5},
			yticklabels={$0$,,,,,$5$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/model_name/aggregate/totals/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m with tuned lens},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/with_tuned_lens/model_name/aggregate/totals/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m with tuned lens},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/with_tuned_lens/model_name/aggregate/totals/pythia-410m-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/with_tuned_lens/model_name/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 3,
					vertical sep=0.25in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Pythia-70m with tuned lens},
			ytick={0.5,1.5,...,5.5},
			yticklabels={$0$,,,,,$5$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/model_name/prompt/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m with tuned lens},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/with_tuned_lens/model_name/prompt/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m with tuned lens},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/with_tuned_lens/model_name/prompt/pythia-410m-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 9,
					vertical sep=0.25in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			ymin=0,
			ymax=6,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick={0.5,1.5,2.5,3.5,4.5,5.5},
			yticklabels={$0$,$1$,$2$,$3$,$4$,$5$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$\ExpansionFactor=1$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x1-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=2$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x2-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=4$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x4-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=8$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x8-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x16-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x32-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x128-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x256-k32.pdf};
	\end{groupplot}
\end{tikzpicture}

==> heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 9,
					vertical sep=0.275in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xmin=0,
			xmax=1,
			ymin=0,
			ymax=6,
			xtick=\empty,
			ytick={0.5,1.5,2.5,3.5,4.5,5.5},
			yticklabels={0,1,2,3,4,5},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$\ExpansionFactor=1$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x1-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=2$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x2-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=4$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x4-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=8$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x8-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x16-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x32-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x128-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x256-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 6,
					vertical sep=0.375in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xmin=0,
			xmax=1,
			xtick=\empty,
			ytick={0.5,1.5,...,5.5},
			yticklabels={$0$,$1$,$2$,$3$,$4$,$5$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$k=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k16.pdf};
		\nextgroupplot[
			title={$k=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$k=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k64.pdf};
		\nextgroupplot[
			title={$k=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k128.pdf};
		\nextgroupplot[
			title={$k=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k256.pdf};
		\nextgroupplot[
			title={$k=512$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k512.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 6,
					vertical sep=0.375in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xmin=0,
			xmax=1,
			xtick=\empty,
			ytick={0.5,1.5,...,5.5},
			yticklabels={$0$,$1$,$2$,$3$,$4$,$5$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$k=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k16.pdf};
		\nextgroupplot[
			title={$k=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$k=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k64.pdf};
		\nextgroupplot[
			title={$k=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k128.pdf};
		\nextgroupplot[
			title={$k=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k256.pdf};
		\nextgroupplot[
			title={$k=512$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/with_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k512.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/gemma2b/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.625in,
			group style={
					group size=1 by 1,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Gemma 2 2B},
			ytick={0.5,1.5,...,25.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,,,$25$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=26,
			] {heatmaps/without_tuned_lens/gemma2b/aggregate/gemma-2-2b-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/gemma2b/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.625in,
			group style={
					group size=1 by 1,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Gemma 2 2B},
			ytick={0.5,1.5,...,25.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,,,$25$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=26,
			] {heatmaps/without_tuned_lens/gemma2b/prompt/gemma-2-2b-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/gpt2/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.625in,
			group style={
					group size=1 by 1,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={GPT-2 small},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/gpt2/aggregate/gpt2-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/gpt2/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.625in,
			group style={
					group size=1 by 1,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={GPT-2 small},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/gpt2/prompt/gpt2-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/llama3b/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.625in,
			group style={
					group size=1 by 1,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Llama 3.2 3B},
			ytick={0.5,1.5,...,27.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,,,,,$27$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=28,
			] {heatmaps/without_tuned_lens/llama3b/aggregate/Llama-3.2-3B-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/llama3b/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.625in,
			group style={
					group size=1 by 1,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Llama 3.2 3B},
			ytick={0.5,1.5,...,27.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,,,,,$27$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=28,
			] {heatmaps/without_tuned_lens/llama3b/prompt/Llama-3.2-3B-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/model_name/aggregate/counts/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 4,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.125)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		% \nextgroupplot[
		% 	title={Pythia-70m},
		% 	ytick={0.5,1.5,...,5.5},
		% 	yticklabels={$0$,,,,,$5$},
		% ]
		% \addplot graphics [
		% 		xmin=0,
		% 		xmax=1,
		% 		ymin=0,
		% 		ymax=6,
		% 	] {heatmaps/without_tuned_lens/model_name/aggregate/counts/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/model_name/aggregate/counts/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/aggregate/counts/pythia-410m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1b},
			ytick={0.5,1.5,...,15.5},
			yticklabels={$0$,,,,,,,,,,,,,,,$15$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=16,
			] {heatmaps/without_tuned_lens/model_name/aggregate/counts/pythia-1b-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1.4b},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/aggregate/counts/pythia-1.4b-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/model_name/aggregate/probs/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 4,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.125)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		% \nextgroupplot[
		% 	title={Pythia-70m},
		% 	ytick={0.5,1.5,...,5.5},
		% 	yticklabels={$0$,,,,,$5$},
		% ]
		% \addplot graphics [
		% 		xmin=0,
		% 		xmax=1,
		% 		ymin=0,
		% 		ymax=6,
		% 	] {heatmaps/without_tuned_lens/model_name/aggregate/probs/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/model_name/aggregate/probs/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/aggregate/probs/pythia-410m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1b},
			ytick={0.5,1.5,...,15.5},
			yticklabels={$0$,,,,,,,,,,,,,,,$15$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=16,
			] {heatmaps/without_tuned_lens/model_name/aggregate/probs/pythia-1b-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1.4b},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/aggregate/probs/pythia-1.4b-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/model_name/aggregate/totals/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 4,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.125)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		% \nextgroupplot[
		% 	title={Pythia-70m},
		% 	ytick={0.5,1.5,...,5.5},
		% 	yticklabels={$0$,,,,,$5$},
		% ]
		% \addplot graphics [
		% 		xmin=0,
		% 		xmax=1,
		% 		ymin=0,
		% 		ymax=6,
		% 	] {heatmaps/without_tuned_lens/model_name/aggregate/totals/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/model_name/aggregate/totals/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/aggregate/totals/pythia-410m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1b},
			ytick={0.5,1.5,...,15.5},
			yticklabels={$0$,,,,,,,,,,,,,,,$15$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=16,
			] {heatmaps/without_tuned_lens/model_name/aggregate/totals/pythia-1b-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1.4b},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/aggregate/totals/pythia-1.4b-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/model_name/prompt/counts/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 4,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.125)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		% \nextgroupplot[
		% 	title={Pythia-70m},
		% 	ytick={0.5,1.5,...,5.5},
		% 	yticklabels={$0$,,,,,$5$},
		% ]
		% \addplot graphics [
		% 		xmin=0,
		% 		xmax=1,
		% 		ymin=0,
		% 		ymax=6,
		% 	] {heatmaps/without_tuned_lens/model_name/prompt/counts/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/model_name/prompt/counts/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/prompt/counts/pythia-410m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1b},
			ytick={0.5,1.5,...,15.5},
			yticklabels={$0$,,,,,,,,,,,,,,,$15$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=16,
			] {heatmaps/without_tuned_lens/model_name/prompt/counts/pythia-1b-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1.4b},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/prompt/counts/pythia-1.4b-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/model_name/prompt/probs/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 4,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.125)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		% \nextgroupplot[
		% 	title={Pythia-70m},
		% 	ytick={0.5,1.5,...,5.5},
		% 	yticklabels={$0$,,,,,$5$},
		% ]
		% \addplot graphics [
		% 		xmin=0,
		% 		xmax=1,
		% 		ymin=0,
		% 		ymax=6,
		% 	] {heatmaps/without_tuned_lens/model_name/prompt/probs/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/model_name/prompt/probs/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/prompt/probs/pythia-410m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1b},
			ytick={0.5,1.5,...,15.5},
			yticklabels={$0$,,,,,,,,,,,,,,,$15$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=16,
			] {heatmaps/without_tuned_lens/model_name/prompt/probs/pythia-1b-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1.4b},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/prompt/probs/pythia-1.4b-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/model_name/prompt/totals/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 4,
					vertical sep=0.225in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.125)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick align=outside,
			tick pos=left,
		]
		% \nextgroupplot[
		% 	title={Pythia-70m},
		% 	ytick={0.5,1.5,...,5.5},
		% 	yticklabels={$0$,,,,,$5$},
		% ]
		% \addplot graphics [
		% 		xmin=0,
		% 		xmax=1,
		% 		ymin=0,
		% 		ymax=6,
		% 	] {heatmaps/without_tuned_lens/model_name/prompt/totals/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-160m},
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/model_name/prompt/totals/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-410m},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/prompt/totals/pythia-410m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1b},
			ytick={0.5,1.5,...,15.5},
			yticklabels={$0$,,,,,,,,,,,,,,,$15$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=16,
			] {heatmaps/without_tuned_lens/model_name/prompt/totals/pythia-1b-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={Pythia-1.4b},
			ytick={0.5,1.5,...,23.5},
			yticklabels={$0$,,,,,,,,,,,,,,,,,,,,,,,$23$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=24,
			] {heatmaps/without_tuned_lens/model_name/prompt/totals/pythia-1.4b-deduped-x64-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 9,
					vertical sep=0.275in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$\ExpansionFactor=1$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/pythia-160m-deduped-x1-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=2$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/pythia-160m-deduped-x2-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=4$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/pythia-160m-deduped-x4-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=8$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/pythia-160m-deduped-x8-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/pythia-160m-deduped-x16-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/pythia-160m-deduped-x32-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/pythia-160m-deduped-x128-k32.pdf};
			\nextgroupplot[
				title={$\ExpansionFactor=256$},
			]
			\addplot graphics [
					xmin=0,
					xmax=1,
					ymin=0,
					ymax=12,
				] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/aggregate/pythia-160m-deduped-x256-k32.pdf};
	\end{groupplot}
\end{tikzpicture}

==> heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 9,
					vertical sep=0.275in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$\ExpansionFactor=1$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/pythia-160m-deduped-x1-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=2$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/pythia-160m-deduped-x2-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=4$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/pythia-160m-deduped-x4-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=8$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/pythia-160m-deduped-x8-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/pythia-160m-deduped-x16-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/pythia-160m-deduped-x32-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/pythia-160m-deduped-x128-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/expansion_factor/prompt/pythia-160m-deduped-x256-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 12,
					vertical sep=0.275in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=768,
			ymin=0,
			ymax=12,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick={0.5,1.5,2.5,3.5,4.5,5.5},
			yticklabels={$0$,$1$,$2$,$3$,$4$,$5$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Trained on layer 0},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l0.pdf};
		\nextgroupplot[
			title={Trained on layer 1},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l1.pdf};
		\nextgroupplot[
			title={Trained on layer 2},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l2.pdf};
		\nextgroupplot[
			title={Trained on layer 3},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l3.pdf};
		\nextgroupplot[
			title={Trained on layer 4},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l4.pdf};
		\nextgroupplot[
			title={Trained on layer 5},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l5.pdf};
		\nextgroupplot[
			title={Trained on layer 6},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l6.pdf};
		\nextgroupplot[
			title={Trained on layer 7},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l7.pdf};
		\nextgroupplot[
			title={Trained on layer 8},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l8.pdf};
		\nextgroupplot[
			title={Trained on layer 9},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l9.pdf};
		\nextgroupplot[
			title={Trained on layer 10},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l10.pdf};
		\nextgroupplot[
			title={Trained on layer 11},
		]
		\addplot graphics [
				xmin=0,
				xmax=768,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/single_layer/aggregate/pythia-160m-deduped-x64-k32-l11.pdf};
	\end{groupplot}
\end{tikzpicture}

==> heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 6,
					vertical sep=0.375in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xmin=0,
			xmax=1,
			xtick=\empty,
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$k=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/aggregate/pythia-160m-deduped-x64-k16.pdf};
		\nextgroupplot[
			title={$k=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/aggregate/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$k=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/aggregate/pythia-160m-deduped-x64-k64.pdf};
		\nextgroupplot[
			title={$k=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/aggregate/pythia-160m-deduped-x64-k128.pdf};
		\nextgroupplot[
			title={$k=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/aggregate/pythia-160m-deduped-x64-k256.pdf};
		\nextgroupplot[
			title={$k=512$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/aggregate/pythia-160m-deduped-x64-k512.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 6,
					vertical sep=0.375in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xmin=0,
			xmax=1,
			xtick=\empty,
			ytick={0.5,1.5,...,11.5},
			yticklabels={$0$,,,,,,,,,,,$11$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$k=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/prompt/pythia-160m-deduped-x64-k16.pdf};
		\nextgroupplot[
			title={$k=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/prompt/pythia-160m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$k=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/prompt/pythia-160m-deduped-x64-k64.pdf};
		\nextgroupplot[
			title={$k=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/prompt/pythia-160m-deduped-x64-k128.pdf};
		\nextgroupplot[
			title={$k=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/prompt/pythia-160m-deduped-x64-k256.pdf};
		\nextgroupplot[
			title={$k=512$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=12,
			] {heatmaps/without_tuned_lens/pythia-160m-deduped/sparsity_k/prompt/pythia-160m-deduped-x64-k512.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 9,
					vertical sep=0.275in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick={0.5,1.5,2.5,3.5,4.5,5.5},
			yticklabels={$0$,$1$,$2$,$3$,$4$,$5$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$\ExpansionFactor=1$},
			xmin=0,
			xmax=512,
		]
		\addplot graphics [
				xmin=0,
				xmax=512,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x1-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=2$},
			xmin=0,
			xmax=1024,
		]
		\addplot graphics [
				xmin=0,
				xmax=1024,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x2-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=4$},
			xmin=0,
			xmax=2048,
		]
		\addplot graphics [
				xmin=0,
				xmax=2048,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x4-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=8$},
			xmin=0,
			xmax=4096,
		]
		\addplot graphics [
				xmin=0,
				xmax=4096,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x8-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=16$},
			xmin=0,
			xmax=8192,
		]
		\addplot graphics [
				xmin=0,
				xmax=8192,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x16-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=32$},
			xmin=0,
			xmax=16384,
		]
		\addplot graphics [
				xmin=0,
				xmax=16384,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x32-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=64$},
			xmin=0,
			xmax=32768,
		]
		\addplot graphics [
				xmin=0,
				xmax=32768,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=128$},
			xmin=0,
			xmax=65536,
		]
		\addplot graphics [
				xmin=0,
				xmax=65536,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x128-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=256$},
			xmin=0,
			xmax=131072,
		]
		\addplot graphics [
				xmin=0,
				xmax=131072,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/aggregate/pythia-70m-deduped-x256-k32.pdf};
	\end{groupplot}
\end{tikzpicture}

==> heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.25in,
			group style={
					group size=1 by 9,
					vertical sep=0.275in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=1,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick={0.5,1.5,2.5,3.5,4.5,5.5},
			yticklabels={0,1,2,3,4,5},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$\ExpansionFactor=1$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x1-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=2$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x2-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=4$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x4-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=8$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x8-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x16-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x32-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x128-k32.pdf};
		\nextgroupplot[
			title={$\ExpansionFactor=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/expansion_factor/prompt/pythia-70m-deduped-x256-k32.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/pythia-70m-deduped/single_layer/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 6,
					vertical sep=0.275in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.1)}},
			enlargelimits=false,
			axis on top,
			xmin=0,
			xmax=512,
			ymin=0,
			ymax=6,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xtick=\empty,
			ytick={0.5,1.5,2.5,3.5,4.5,5.5},
			yticklabels={$0$,$1$,$2$,$3$,$4$,$5$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={Trained on layer 0},
		]
		\addplot graphics [
				xmin=0,
				xmax=512,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/single_layer/aggregate/pythia-70m-deduped-x64-k32-l0.pdf};
		\nextgroupplot[
			title={Trained on layer 1},
		]
		\addplot graphics [
				xmin=0,
				xmax=512,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/single_layer/aggregate/pythia-70m-deduped-x64-k32-l1.pdf};
		\nextgroupplot[
			title={Trained on layer 2},
		]
		\addplot graphics [
				xmin=0,
				xmax=512,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/single_layer/aggregate/pythia-70m-deduped-x64-k32-l2.pdf};
		\nextgroupplot[
			title={Trained on layer 3},
		]
		\addplot graphics [
				xmin=0,
				xmax=512,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/single_layer/aggregate/pythia-70m-deduped-x64-k32-l3.pdf};
		\nextgroupplot[
			title={Trained on layer 4},
		]
		\addplot graphics [
				xmin=0,
				xmax=512,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/single_layer/aggregate/pythia-70m-deduped-x64-k32-l4.pdf};
		\nextgroupplot[
			title={Trained on layer 5},
		]
		\addplot graphics [
				xmin=0,
				xmax=512,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/single_layer/aggregate/pythia-70m-deduped-x64-k32-l5.pdf};
	\end{groupplot}
\end{tikzpicture}

==> heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 6,
					vertical sep=0.375in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xmin=0,
			xmax=1,
			xtick=\empty,
			ytick={0.5,1.5,...,5.5},
			yticklabels={$0$,$1$,$2$,$3$,$4$,$5$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$k=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k16.pdf};
		\nextgroupplot[
			title={$k=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$k=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k64.pdf};
		\nextgroupplot[
			title={$k=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k128.pdf};
		\nextgroupplot[
			title={$k=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k256.pdf};
		\nextgroupplot[
			title={$k=512$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/aggregate/pythia-70m-deduped-x64-k512.pdf};
	\end{groupplot}
\end{tikzpicture}


==> heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			width=5.5in,
			height=1.5in,
			group style={
					group size=1 by 6,
					vertical sep=0.375in,
					xlabels at=edge bottom,
				},
			title style={font=\small},
			every axis title/.style={at={(0.5,1.15)}},
			enlargelimits=false,
			axis on top,
			xlabel={Latent},
			ylabel={Layer},
			y label style={anchor=south,at={(axis description cs:-0.05,.5)}},
			xmin=0,
			xmax=1,
			xtick=\empty,
			ytick={0.5,1.5,...,5.5},
			yticklabels={$0$,$1$,$2$,$3$,$4$,$5$},
			ytick align=outside,
			tick pos=left,
		]
		\nextgroupplot[
			title={$k=16$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k16.pdf};
		\nextgroupplot[
			title={$k=32$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k32.pdf};
		\nextgroupplot[
			title={$k=64$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k64.pdf};
		\nextgroupplot[
			title={$k=128$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k128.pdf};
		\nextgroupplot[
			title={$k=256$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k256.pdf};
		\nextgroupplot[
			title={$k=512$},
		]
		\addplot graphics [
				xmin=0,
				xmax=1,
				ymin=0,
				ymax=6,
			] {heatmaps/without_tuned_lens/pythia-70m-deduped/sparsity_k/prompt/pythia-70m-deduped-x64-k512.pdf};
	\end{groupplot}
\end{tikzpicture}


==> mmcs/figure.tex <==
\newcommand{\addplotmmcs}[2]{
	\addplot+ [
		mark=*,error bars/.cd,y dir=both, y explicit,
	] table [
			col sep=comma,
			x={#1},
			y=mean,
			y error=sem,
		] {#2}
}
\begin{tikzpicture}
	\begin{groupplot}[
			scale only axis,
			width=2in,
			height=2in,
			group style={
					group size=2 by 1,
					horizontal sep=0.25in,
					y descriptions at=edge left,
				},
			xmode=log,
			ymin=0.125,
			ymax=0.32,
			title style={
					anchor=north,
					at={(0.5,1.1)},
					font=\small
				},
			ylabel={Mean Max Cosine Similarity},
			y label style={anchor=south,at={(-0.2,0.5)}},
			grid=major,
			cycle list/Paired,
			legend cell align={left},
			legend columns=2,
			legend style={
					anchor=south,
					at={(0,-0.75)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
			every axis plot/.append={
					error bar style={line width=0.75pt},
					error mark options={
							line width=0.75pt,
							mark size=2pt,
							rotate=90,
						},
				}
		]
		\nextgroupplot[
			title={Sparsity $k=32$},
			xlabel={Expansion Factor $\ExpansionFactor$},
			xmin=0.5,
			xmax=512,
		]
		\addplotmmcs{expansion_factor}{mmcs/pythia-70m-deduped/expansion_factor.csv};
		\addplotmmcs{expansion_factor}{mmcs/pythia-70m-deduped-lens/expansion_factor.csv};
		\addplotmmcs{expansion_factor}{mmcs/pythia-160m-deduped/expansion_factor.csv};
		\addplotmmcs{expansion_factor}{mmcs/pythia-160m-deduped-lens.csv};
		\addplotmmcs{expansion_factor}{mmcs/pythia-410m-deduped.csv};
		\addplotmmcs{expansion_factor}{mmcs/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotmmcs{expansion_factor}{mmcs/pythia-1b-deduped.csv};
		\addplotmmcs{expansion_factor}{mmcs/pythia-1.4b-deduped.csv};
		\addplotmmcs{expansion_factor}{mmcs/gemma2b.csv};
		\addplotmmcs{expansion_factor}{mmcs/llama3b.csv};
		\addplotmmcs{expansion_factor}{mmcs/gpt2.csv};
		\draw[dashed,gray] (axis cs:64,0) -- (axis cs:64,1);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
		]
		\addplotmmcs{k}{mmcs/pythia-70m-deduped/sparsity_k.csv};
		\addplotmmcs{k}{mmcs/pythia-70m-deduped-lens/sparsity_k.csv};
		\addplotmmcs{k}{mmcs/pythia-160m-deduped/sparsity_k.csv};
		\addplotmmcs{k}{mmcs/pythia-160m-deduped-lens.csv};
		\addplotmmcs{k}{mmcs/pythia-410m-deduped.csv};
		\addplotmmcs{k}{mmcs/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotmmcs{k}{mmcs/pythia-1b-deduped.csv};
		\addplotmmcs{k}{mmcs/pythia-1.4b-deduped.csv};
		\addplotmmcs{k}{mmcs/gemma2b.csv};
		\addplotmmcs{k}{mmcs/llama3b.csv};
		\addplotmmcs{k}{mmcs/gpt2.csv};
		\draw[dashed,gray] (axis cs:32,0) -- (axis cs:32,1);
		\addlegendentry{Pythia-70m}
		\addlegendentry{Pythia-70m with tuned lens}
		\addlegendentry{Pythia-160m}
		\addlegendentry{Pythia-160m with tuned lens}
		\addlegendentry{Pythia-410m}
		\addlegendentry{Pythia-410m with tuned lens}
		\addlegendentry{Pythia-1b}
		\addlegendentry{Pythia-1.4b}
		\addlegendentry{Gemma 2 2B}
		\addlegendentry{Llama 3.2 3B}
		\addlegendentry{GPT-2 small}
	\end{groupplot}
\end{tikzpicture}


==> num_layers/figure.tex <==
\newcommand{\addplotnl}[2]{
	\addplot+ [mark=*] table [
			col sep=comma,
			x=#1,
			y=rel,
		]{#2}
}
\newcommand{\addplotnlx}[1]{
	\addplotnl{expansion_factor}{#1}
}
\newcommand{\addplotnlk}[1]{
	\addplotnl{k}{#1}
}
\begin{tikzpicture}
	\begin{groupplot}[
			scale only axis,
			width=2in,
			height=2in,
			group style={
					group size=2 by 1,
					horizontal sep=0.125in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			cycle list/Paired,
			title style={
					anchor=north,
					at={(0.5,1.1)},
					font=\small
				},
			y label style={
					anchor=south,
					at={(-0.2,.5)},
					font=\large,
				},
			ymin=2e-4,
			ymax=1.5,
			xmode=log,
			ymode=log,
			grid=major,
			legend cell align={left},
			legend columns=2,
			legend style={
					anchor=south,
					at={(0,-0.75)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\nextgroupplot[
			title={Sparsity $k=32$},
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={\Large $\frac{\text{Mean Active Layers}}{\text{Total Layers}}$},
			xmin=0.5,
			xmax=512,
		]
		\addplotnlx{num_layers/pythia-70m-deduped/expansion_factor.csv};
		\addplotnlx{num_layers/pythia-70m-deduped-lens/expansion_factor.csv};
		\addplotnlx{num_layers/pythia-160m-deduped/expansion_factor.csv};
		\addplotnlx{num_layers/pythia-160m-deduped-lens.csv};
		\addplotnlx{num_layers/pythia-410m-deduped.csv};
		\addplotnlx{num_layers/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotnlx{num_layers/pythia-1b-deduped.csv};
		\addplotnlx{num_layers/pythia-1.4b-deduped.csv};
		\addplotnlx{num_layers/gemma2b.csv};
		\addplotnlx{num_layers/llama3b.csv};
		\addplotnlx{num_layers/gpt2.csv};
		\draw[dashed,gray] (axis cs:64,2e-4) -- (axis cs:64,1.5);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
		]
		\addplotnlk{num_layers/pythia-70m-deduped/sparsity_k.csv};
		\addplotnlk{num_layers/pythia-70m-deduped-lens/sparsity_k.csv};
		\addplotnlk{num_layers/pythia-160m-deduped/sparsity_k.csv};
		\addplotnlk{num_layers/pythia-160m-deduped-lens.csv};
		\addplotnlk{num_layers/pythia-410m-deduped.csv};
		\addplotnlk{num_layers/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotnlk{num_layers/pythia-1b-deduped.csv};
		\addplotnlk{num_layers/pythia-1.4b-deduped.csv};
		\addplotnlk{num_layers/gemma2b.csv};
		\addplotnlk{num_layers/llama3b.csv};
		\addplotnlk{num_layers/gpt2.csv};
		\draw[dashed,gray] (axis cs:32,2e-4) -- (axis cs:32,1.5);
		\addlegendentry{Pythia-70m}
		\addlegendentry{Pythia-70m with tuned lens}
		\addlegendentry{Pythia-160m}
		\addlegendentry{Pythia-160m with tuned lens}
		\addlegendentry{Pythia-410m}
		\addlegendentry{Pythia-410m with tuned lens}
		\addlegendentry{Pythia-1b}
		\addlegendentry{Pythia-1.4b}
		\addlegendentry{Gemma 2 2B}
		\addlegendentry{Llama 3.2 3B}
		\addlegendentry{GPT-2 small}
	\end{groupplot}
\end{tikzpicture}


==> num_layers/model_name/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			scale only axis,
			width=4.5in,
			height=1.5in,
			group style={
					group size=1 by 2,
					vertical sep=0.75in,
				},
			xbar,
			xticklabel style={/pgf/number format/fixed},
			y dir=reverse,
			enlarge y limits=true,
			symbolic y coords={
					Pythia-70m,
					Pythia-160m,
					Pythia-410m,
					Pythia-1b,
					Pythia-1.4b,
					gemma-2-2b,
					Llama-3.2-3B,
					gpt2,
				},
			ytick=data,
			yticklabels={
					Pythia-70m,
					Pythia-160m,
					Pythia-410m,
					Pythia-1b,
					Pythia-1.4b,
					Gemma 2 2B,
					Llama 3.2 3B,
					GPT-2 small
				},
			xtick align=outside,
			ytick align=outside,
			tick pos=left,
			axis x line*=left,
			axis y line*=left,
			axis line style=semithick,
			every tick/.style={black,semithick},
			legend cell align={left},
			legend columns=1,
			legend style={
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\nextgroupplot[
			xlabel={Mean Active Layers / Total Layers},
			xmin=0,
			xmax=0.2,
			bar width=0.0375in,
			legend pos=south east,
		]
		\addplot+ [Paired-A] table [
				col sep=comma,
				y=model_name,
				x=rel,
			]{num_layers/model_name/without_tuned_lens.csv};
		\addplot+ [Paired-B] table [
				col sep=comma,
				y=model_name,
				x=rel,
			]{num_layers/model_name/with_tuned_lens.csv};
		\addlegendentry{Standard}
		\addlegendentry{Tuned lens}
	\end{groupplot}
\end{tikzpicture}

==> resid_cos_sim/figure.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{axis}[
			scale only axis,
			width=4.5in,
			height=1.25in,
			cycle list={[colors of colormap={1000,850,...,150}]},
			xlabel={Relative Layer},
			ylabel={Mean Cosine Similarity},
			y label style={anchor=south,at={(-0.075,.5)}},
			xmin=0,
			xmax=1,
			ymin=0,
			ymax=1,
			enlarge x limits=0.05,
			xtick align=outside,
			ytick align=outside,
			tick pos=left,
			legend cell align={left},
			legend columns=2,
			legend pos=south west,
			legend style={
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/4,
				y=mean,
				y error=sem,
			]{resid_cos_sim/pythia-70m-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/10,
				y=mean,
				y error=sem,
			]{resid_cos_sim/pythia-160m-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/22,
				y=mean,
				y error=sem,
			]{resid_cos_sim/pythia-410m-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/14,
				y=mean,
				y error=sem,
			]{resid_cos_sim/pythia-1b-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/22,
				y=mean,
				y error=sem,
			]{resid_cos_sim/pythia-1.4b-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/30,
				y=mean,
				y error=sem,
			]{resid_cos_sim/pythia-2.8b-deduped.csv};
		\addlegendentry{Pythia-70m}
		\addlegendentry{Pythia-160m}
		\addlegendentry{Pythia-410m}
		\addlegendentry{Pythia-1b}
		\addlegendentry{Pythia-1.4b}
		\addlegendentry{Pythia-2.8b}
	\end{axis}
\end{tikzpicture}


==> resid_l2_norm/figure.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{axis}[
			scale only axis,
			width=4.5in,
			height=1.5in,
			cycle list={[colors of colormap={1000,850,...,150}]},
			xlabel={Relative Layer},
			ylabel={Mean $L^2$ Norm},
			y label style={anchor=south,at={(-0.075,.5)}},
			xmin=0,
			xmax=1,
			enlarge x limits=0.05,
			xtick align=outside,
			ytick align=outside,
			tick pos=left,
			legend cell align={left},
			legend columns=2,
			legend pos=north west,
			legend style={
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/5,
				y=mean,
				y error=sem,
			]{resid_l2_norm/pythia-70m-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/11,
				y=mean,
				y error=sem,
			]{resid_l2_norm/pythia-160m-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/23,
				y=mean,
				y error=sem,
			]{resid_l2_norm/pythia-410m-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/15,
				y=mean,
				y error=sem,
			]{resid_l2_norm/pythia-1b-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/23,
				y=mean,
				y error=sem,
			]{resid_l2_norm/pythia-1.4b-deduped.csv};
		\addplot+ [mark=*,mark size=1.5pt,error bars/.cd,y dir=both, y explicit] table [
				col sep=comma,
				x expr=\thisrowno{0}/31,
				y=mean,
				y error=sem,
			]{resid_l2_norm/pythia-2.8b-deduped.csv};
		\addlegendentry{Pythia-70m}
		\addlegendentry{Pythia-160m}
		\addlegendentry{Pythia-410m}
		\addlegendentry{Pythia-1b}
		\addlegendentry{Pythia-1.4b}
		\addlegendentry{Pythia-2.8b}
	\end{axis}
\end{tikzpicture}


==> test/dead_latents/figure.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{groupplot}[
			scale only axis,
			width=3.75in,
			height=0.8in,
			group style={
					group size=1 by 3,
					vertical sep=0.25in,
					x descriptions at=edge bottom,
				},
			cycle list={[colors of colormap={1000,900,...,0}]},
			xlabel={Number of Tokens $\NumTokens$},
			y label style={
					anchor=south,
					at={(axis description cs:-0.1,.5)},
				},
			xmin=0,
			xmax=1e9,
			scaled x ticks=false,
			ymin=0,
			grid=major,
			legend cell align={left},
			legend columns=1,
			legend style={
					anchor=west,
					at={(1.035,0.5)},
					column sep=0in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\nextgroupplot[
			ylabel={Layer 5 FVU},
			ymax=0.15,
			yticklabel style={
					/pgf/number format/fixed
				},
			scaled y ticks=false,
		]
		\pgfplotstableread[col sep=comma]{test/dead_latents/train_fvu_layer_5.csv}\Data
		\pgfplotsinvokeforeach{512,1024,2048,4096,8192,16384,32768,65536,131072}{
			\addplot table [x=tokens,y={n = #1},mark=none] {\Data};
		}
		\nextgroupplot[
			ylabel=Auxiliary Loss,
			yticklabel style={
					/pgf/number format/fixed
				},
			scaled y ticks=false,
		]
		\pgfplotstableread[col sep=comma]{test/dead_latents/loss_auxk.csv}\Data
		\pgfplotsinvokeforeach{512,1024,2048,4096,8192,16384,32768,65536,131072}{
			\addplot table [x=tokens,y={n = #1},mark=none] {\Data};
		}
		\addlegendentry{{$\ExpansionFactor = 1$}}
		\addlegendentry{{$\ExpansionFactor = 2$}}
		\addlegendentry{{$\ExpansionFactor = 4$}}
		\addlegendentry{{$\ExpansionFactor = 8$}}
		\addlegendentry{{$\ExpansionFactor = 16$}}
		\addlegendentry{{$\ExpansionFactor = 32$}}
		\addlegendentry{{$\ExpansionFactor = 64$}}
		\addlegendentry{{$\ExpansionFactor = 128$}}
		\addlegendentry{{$\ExpansionFactor = 256$}}
		\nextgroupplot[
			ylabel=Dead Latents,
			xtick={0,100000000,...,1000000000},
			xticklabels={
					0,,
					\num{2e8},,
					\num{4e8},,
					\num{6e8},,
					\num{8e8},,
					\num{1e9}
				},
			ytick={0,0.05,0.1},
			yticklabels={$0$,$5$\%,$10$\%},
		]
		\pgfplotstableread[col sep=comma]{test/dead_latents/train_dead_abs.csv}\Data
		\pgfplotsinvokeforeach{512,1024,2048,4096,8192,16384,32768,65536,131072}{
			\addplot table [x=tokens,y={n = #1},mark=none] {\Data};
		}
	\end{groupplot}
\end{tikzpicture}

==> test/pythia-160m-deduped-layer/figure.tex <==
\newcommand{\maxfvu}{1.349}
\newcommand{\maxloss}{8.726}
\begin{tikzpicture}
	\pgfplotsset{
		colormap/RdYlGn,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.95in,
			height=1.95in,
			group style={
					group size=2 by 2,
					horizontal sep=0.625in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			enlargelimits=false,
			colormap={reverse RdYlGn}{
					indices of colormap={
							\pgfplotscolormaplastindexof{RdYlGn},...,0 of RdYlGn}
				},
			every axis title/.style={at={(0.5,1.075)}},
			xlabel={Test Layer},
			ylabel={Single-Layer SAEs},
			y label style={anchor=south,at={(axis description cs:-0.1,.5)}},
			xtick={0,1,...,11},
			xticklabels={0,1,...,11},
			xtick align=outside,
			ytick={0,1,...,11},
			yticklabels={0,1,...,11},
			ytick align=outside,
			major tick length=0,
		]
		\nextgroupplot[
			title={FVU},
			point meta min=0,
			point meta max=\maxfvu,
			colorbar right,
			colorbar style={
					width=0.1in,
				}
		]
		\addplot[
			matrix plot,
			mesh/cols=11,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-160m-deduped-layer/single_layer/fvu.csv};
		\nextgroupplot[
			title={Delta Cross-Entropy Loss},
			point meta min=0,
			point meta max=\maxloss,
			colorbar right,
			colorbar style={
					width=0.1in,
				}
		]
		\addplot[
			matrix plot,
			mesh/cols=11,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-160m-deduped-layer/single_layer/loss.csv};
		\nextgroupplot[
			point meta min=0,
			point meta max=\maxfvu,
			height=0.1625in,
			ylabel={MLSAE},
			ytick=\empty,
			ymax=0.5,
		]
		\addplot[
			matrix plot,
			mesh/cols=11,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-160m-deduped-layer/multi_layer/fvu.csv};
		\nextgroupplot[
			point meta min=0,
			point meta max=\maxloss,
			height=0.1625in,
			ymax=0.5,
		]
		\addplot[
			matrix plot,
			mesh/cols=11,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-160m-deduped-layer/multi_layer/loss.csv};
	\end{groupplot}
\end{tikzpicture}

==> test/pythia-160m-deduped/downstream_loss.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.875in,
			height=1.375in,
			group style={
					group size=2 by 2,
					horizontal sep=0.125in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			cycle list={[colors of colormap={1000,925,...,75}]},
			title style={
					anchor=north,
					at={(0.5,1.1)},
					font=\small
				},
			xmode=log,
			ymode=log,
			grid=major,
			legend cell align={left},
			legend columns=1,
			legend style={
					anchor=west,
					at={(1.05,1)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\pgfplotstableread[col sep=comma]{test/pythia-160m-deduped/expansion_factor.csv}\ExpansionFactorCSV
		\pgfplotstableread[col sep=comma]{test/pythia-160m-deduped/sparsity_k.csv}\SparsityKCSV
		\nextgroupplot[
			title={Sparsity $k=32$},
			ylabel={Delta CE loss},
			y label style={anchor=south,at={(-0.2,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=0.03,
			ymax=5,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_5] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_6] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_7] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_8] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_9] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_10] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_11] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=val/loss/delta/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,0.03) -- (axis cs:64,5);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xmin=1e1,
			xmax=1e3,
			ymin=0.03,
			ymax=5,
		]
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_5] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_6] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_7] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_8] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_9] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_10] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_11] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=val/loss/delta/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,0.03) -- (axis cs:32,5);
		\nextgroupplot[
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={KL divergence},
			y label style={anchor=south,at={(-0.2,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=100,
			ymax=12500,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_5] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_6] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_7] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_8] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_9] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_10] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_11] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=val/logit/kldiv/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,100) -- (axis cs:64,12500);
		\nextgroupplot[
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
			ymin=100,
			ymax=12500,
		]
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_5] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_6] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_7] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_8] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_9] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_10] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_11] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=val/logit/kldiv/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,100) -- (axis cs:32,12500);
		\addlegendentry{Layer 0}
		\addlegendentry{Layer 1}
		\addlegendentry{Layer 2}
		\addlegendentry{Layer 3}
		\addlegendentry{Layer 4}
		\addlegendentry{Layer 5}
		\addlegendentry{Layer 6}
		\addlegendentry{Layer 7}
		\addlegendentry{Layer 8}
		\addlegendentry{Layer 9}
		\addlegendentry{Layer 10}
		\addlegendentry{Layer 11}
		\addlegendentry{Mean}
	\end{groupplot}
\end{tikzpicture}

==> test/pythia-160m-deduped/l1_norm.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.875in,
			height=2.75in,
			group style={
					group size=2 by 1,
					horizontal sep=0.35in,
					x descriptions at=edge bottom,
				},
			cycle list={[colors of colormap={1000,925,...,75}]},
			title style={
					anchor=north,
					at={(0.5,1.075)},
					font=\small
				},
			xmode=log,
			ymode=log,
			grid=major,
			legend cell align={left},
			legend columns=1,
			legend style={
					anchor=west,
					at={(1.05,0.5)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\pgfplotstableread[col sep=comma]{test/pythia-160m-deduped/expansion_factor.csv}\ExpansionFactorCSV
		\pgfplotstableread[col sep=comma]{test/pythia-160m-deduped/sparsity_k.csv}\SparsityKCSV
		\nextgroupplot[
			title={Sparsity $k=32$},
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={$L^1$ norm},
			y label style={anchor=south,at={(axis description cs:-0.125,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=60,
			ymax=120,
			ytick={60,80,...,120},
			yticklabels={$60$,$80$,$100$,$120$},
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_5] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_6] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_7] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_8] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_9] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_10] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_11] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=train/l1/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,60) -- (axis cs:64,120);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
			ymin=40,
			ymax=1e3,
		]
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_5] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_6] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_7] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_8] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_9] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_10] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_11] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=train/l1/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,40) -- (axis cs:32,1e3);
		\addlegendentry{Layer 0}
		\addlegendentry{Layer 1}
		\addlegendentry{Layer 2}
		\addlegendentry{Layer 3}
		\addlegendentry{Layer 4}
		\addlegendentry{Layer 5}
		\addlegendentry{Layer 6}
		\addlegendentry{Layer 7}
		\addlegendentry{Layer 8}
		\addlegendentry{Layer 9}
		\addlegendentry{Layer 10}
		\addlegendentry{Layer 11}
		\addlegendentry{Mean}
	\end{groupplot}
\end{tikzpicture}

==> test/pythia-160m-deduped/reconstruction_error.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.875in,
			height=1.375in,
			group style={
					group size=2 by 2,
					horizontal sep=0.125in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			cycle list={[colors of colormap={1000,925,...,75}]},
			title style={
					anchor=north,
					at={(0.5,1.1)},
					font=\small
				},
			xmode=log,
			ymode=log,
			grid=major,
			legend cell align={left},
			legend columns=1,
			legend style={
					anchor=west,
					at={(1.05,1)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\pgfplotstableread[col sep=comma]{test/pythia-160m-deduped/expansion_factor.csv}\ExpansionFactorCSV
		\pgfplotstableread[col sep=comma]{test/pythia-160m-deduped/sparsity_k.csv}\SparsityKCSV
		\nextgroupplot[
			title={Sparsity $k=32$},
			ylabel={FVU},
			y label style={anchor=south,at={(-0.2,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=0.025,
			ymax=0.375,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_5] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_6] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_7] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_8] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_9] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_10] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_11] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=train/fvu/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,0.025) -- (axis cs:64,0.375);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xmin=1e1,
			xmax=1e3,
			ymin=0.025,
			ymax=0.375,
		]
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_5] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_6] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_7] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_8] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_9] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_10] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_11] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=train/fvu/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,0.025) -- (axis cs:32,375);
		\nextgroupplot[
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={MSE},
			y label style={anchor=south,at={(-0.2,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=0.002,
			ymax=1.5,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_5] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_6] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_7] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_8] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_9] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_10] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_11] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=train/mse/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,0.002) -- (axis cs:64,1.5);
		\nextgroupplot[
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
			ymin=0.002,
			ymax=1.5,
		]
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_5] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_6] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_7] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_8] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_9] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_10] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_11] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=train/mse/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,0.002) -- (axis cs:32,1.5);
		\addlegendentry{Layer 0}
		\addlegendentry{Layer 1}
		\addlegendentry{Layer 2}
		\addlegendentry{Layer 3}
		\addlegendentry{Layer 4}
		\addlegendentry{Layer 5}
		\addlegendentry{Layer 6}
		\addlegendentry{Layer 7}
		\addlegendentry{Layer 8}
		\addlegendentry{Layer 9}
		\addlegendentry{Layer 10}
		\addlegendentry{Layer 11}
		\addlegendentry{Mean}
	\end{groupplot}
\end{tikzpicture}


==> test/pythia-410m-deduped-layer/figure.tex <==
\newcommand{\maxfvu}{1.787}
\newcommand{\maxloss}{9.333}
\newcommand{\maxlayers}{23}
\begin{tikzpicture}
	\pgfplotsset{
		colormap/RdYlGn,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.95in,
			height=1.95in,
			group style={
					group size=2 by 2,
					horizontal sep=0.625in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			enlargelimits=false,
			colormap={reverse RdYlGn}{
					indices of colormap={
							\pgfplotscolormaplastindexof{RdYlGn},...,0 of RdYlGn}
				},
			every axis title/.style={at={(0.5,1.075)}},
			xlabel={Test Layer},
			ylabel={Single-Layer SAEs},
			y label style={anchor=south,at={(axis description cs:-0.1,.5)}},
			xtick={0,2,...,\maxlayers},
			xticklabels={0,2,...,\maxlayers},
			xtick align=outside,
			ytick={0,2,...,\maxlayers},
			yticklabels={0,2,...,\maxlayers},
			ytick align=outside,
			major tick length=0,
		]
		\nextgroupplot[
			title={FVU},
			point meta min=0,
			point meta max=\maxfvu,
			colorbar right,
			colorbar style={
					width=0.1in,
					nodes near coords={},
				}
		]
		\addplot[
			matrix plot,
			mesh/cols=\maxlayers,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-410m-deduped-layer/single_layer/fvu.csv};
		\nextgroupplot[
			title={Delta Cross-Entropy Loss},
			point meta min=0,
			point meta max=\maxloss,
			colorbar right,
			colorbar style={
					width=0.1in,
					nodes near coords={},
				}
		]
		\addplot[
			matrix plot,
			mesh/cols=\maxlayers,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-410m-deduped-layer/single_layer/loss.csv};
		\nextgroupplot[
			point meta min=0,
			point meta max=\maxfvu,
			height=0.08125in,
			ylabel={MLSAE},
			ytick=\empty,
			ymax=0.5,
		]
		\addplot[
			matrix plot,
			mesh/cols=\maxlayers,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-410m-deduped-layer/multi_layer/fvu.csv};
		\nextgroupplot[
			point meta min=0,
			point meta max=\maxloss,
			height=0.08125in,
			ymax=0.5,
		]
		\addplot[
			matrix plot,
			mesh/cols=\maxlayers,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-410m-deduped-layer/multi_layer/loss.csv};
	\end{groupplot}
\end{tikzpicture}

==> test/pythia-70m-deduped-layer/figure.tex <==
\newcommand{\maxfvu}{0.865}
\newcommand{\maxloss}{4.466}
\begin{tikzpicture}
	\pgfplotsset{
		colormap/RdYlGn,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.95in,
			height=1.95in,
			group style={
					group size=2 by 2,
					horizontal sep=0.625in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			enlargelimits=false,
			colormap={reverse RdYlGn}{
					indices of colormap={
							\pgfplotscolormaplastindexof{RdYlGn},...,0 of RdYlGn}
				},
			every axis title/.style={at={(0.5,1.075)}},
			xlabel={Test Layer},
			ylabel={Single-Layer SAEs},
			y label style={anchor=south,at={(axis description cs:-0.1,.5)}},
			xtick={0,1,2,3,4,5},
			xticklabels={0,1,2,3,4,5},
			xtick align=outside,
			ytick={0,1,2,3,4,5},
			yticklabels={0,1,2,3,4,5},
			ytick align=outside,
			major tick length=0,
			nodes near coords={\pgfmathprintnumber[fixed,fixed zerofill,precision=3]{\pgfplotspointmeta}},
			nodes near coords dual threshold/.style args={#1 and #2}{
					small value/.style={
							font=\footnotesize,
							yshift=-6.5pt,
							text=white,
						},
					medium value/.style={
							font=\footnotesize,
							yshift=-6.5pt,
							text=black,
						},
					large value/.style={
							font=\footnotesize,
							yshift=-6.5pt,
							text=white,
						},
					every node near coord/.style={
							check for thresholds/.code={
									\pgfmathfloatifflags{\pgfplotspointmeta}{0}{
										\pgfkeys{/tikz/coordinate}
									}{
										\begingroup
										\pgfkeys{/pgf/fpu}
										\pgfmathparse{\pgfplotspointmeta<#1}
										\global\let\resultlower=\pgfmathresult
										\pgfmathparse{\pgfplotspointmeta>#2}
										\global\let\resultupper=\pgfmathresult
										\endgroup
										\pgfmathfloatcreate{1}{1.0}{0}
										\let\ONE=\pgfmathresult
										\ifx\resultlower\ONE
											\pgfkeysalso{/pgfplots/small value}
										\else
											\ifx\resultupper\ONE
												\pgfkeysalso{/pgfplots/large value}
											\else
												\pgfkeysalso{/pgfplots/medium value}
											\fi
										\fi
									}
								},
							check for thresholds,
						},
				},
			nodes near coords style={
					font=\footnotesize,
					every node/.append style={
							text=black,
						}
				},
			every node near coord/.append style={yshift=-6.5pt}
		]
		\nextgroupplot[
			title={FVU},
			point meta min=0,
			point meta max=\maxfvu,
			nodes near coords dual threshold={0.15 and 0.75},
			colorbar right,
			colorbar style={
					width=0.1in,
					nodes near coords={},
				}
		]
		\addplot[
			matrix plot,
			mesh/cols=5,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-70m-deduped-layer/single_layer/fvu.csv};
		\nextgroupplot[
			title={Delta Cross-Entropy Loss},
			point meta min=0,
			point meta max=\maxloss,
			nodes near coords dual threshold={0.75 and 4},
			colorbar right,
			colorbar style={
					width=0.1in,
					nodes near coords={},
				}
		]
		\addplot[
			matrix plot,
			mesh/cols=5,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-70m-deduped-layer/single_layer/loss.csv};
		\nextgroupplot[
			point meta min=0,
			point meta max=\maxfvu,
			nodes near coords dual threshold={0.15 and 0.75},
			height=0.325in,
			ylabel={MLSAE},
			ytick=\empty,
			ymax=0.5,
		]
		\addplot[
			matrix plot,
			mesh/cols=5,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-70m-deduped-layer/multi_layer/fvu.csv};
		\nextgroupplot[
			point meta min=0,
			point meta max=\maxloss,
			nodes near coords dual threshold={0.75 and 4},
			height=0.325in,
			ymax=0.5,
		]
		\addplot[
			matrix plot,
			mesh/cols=5,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-70m-deduped-layer/multi_layer/loss.csv};
	\end{groupplot}
\end{tikzpicture}

==> test/pythia-70m-deduped-lens-layer/figure.tex <==
\newcommand{\maxfvu}{0.867}
\newcommand{\maxloss}{8.728}
\begin{tikzpicture}
	\pgfplotsset{
		colormap/RdYlGn,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.95in,
			height=1.95in,
			group style={
					group size=2 by 2,
					horizontal sep=0.625in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			enlargelimits=false,
			colormap={reverse RdYlGn}{
					indices of colormap={
							\pgfplotscolormaplastindexof{RdYlGn},...,0 of RdYlGn}
				},
			every axis title/.style={at={(0.5,1.075)}},
			xlabel={Test Layer},
			ylabel={Single-Layer SAEs},
			y label style={anchor=south,at={(axis description cs:-0.1,.5)}},
			xtick={0,1,2,3,4,5},
			xticklabels={0,1,2,3,4,5},
			xtick align=outside,
			ytick={0,1,2,3,4,5},
			yticklabels={0,1,2,3,4,5},
			ytick align=outside,
			major tick length=0,
			nodes near coords={\pgfmathprintnumber[fixed,fixed zerofill,precision=3]{\pgfplotspointmeta}},
			nodes near coords dual threshold/.style args={#1 and #2}{
					small value/.style={
							font=\footnotesize,
							yshift=-6.5pt,
							text=white,
						},
					medium value/.style={
							font=\footnotesize,
							yshift=-6.5pt,
							text=black,
						},
					large value/.style={
							font=\footnotesize,
							yshift=-6.5pt,
							text=white,
						},
					every node near coord/.style={
							check for thresholds/.code={
									\pgfmathfloatifflags{\pgfplotspointmeta}{0}{
										\pgfkeys{/tikz/coordinate}
									}{
										\begingroup
										\pgfkeys{/pgf/fpu}
										\pgfmathparse{\pgfplotspointmeta<#1}
										\global\let\resultlower=\pgfmathresult
										\pgfmathparse{\pgfplotspointmeta>#2}
										\global\let\resultupper=\pgfmathresult
										\endgroup
										\pgfmathfloatcreate{1}{1.0}{0}
										\let\ONE=\pgfmathresult
										\ifx\resultlower\ONE
											\pgfkeysalso{/pgfplots/small value}
										\else
											\ifx\resultupper\ONE
												\pgfkeysalso{/pgfplots/large value}
											\else
												\pgfkeysalso{/pgfplots/medium value}
											\fi
										\fi
									}
								},
							check for thresholds,
						},
				},
			nodes near coords style={
					font=\footnotesize,
					every node/.append style={
							text=black,
						}
				},
			every node near coord/.append style={yshift=-6.5pt}
		]
		\nextgroupplot[
			title={FVU},
			point meta min=0,
			point meta max=\maxfvu,
			nodes near coords dual threshold={0.15 and 0.75},
			colorbar right,
			colorbar style={
					width=0.1in,
					nodes near coords={},
				}
		]
		\addplot[
			matrix plot,
			mesh/cols=5,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-70m-deduped-lens-layer/single_layer/fvu.csv};
		\nextgroupplot[
			title={Delta Cross-Entropy Loss},
			point meta min=0,
			point meta max=\maxloss,
			nodes near coords dual threshold={1.5 and 7},
			colorbar right,
			colorbar style={
					width=0.1in,
					nodes near coords={},
				}
		]
		\addplot[
			matrix plot,
			mesh/cols=5,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-70m-deduped-lens-layer/single_layer/loss.csv};
		\nextgroupplot[
			point meta min=0,
			point meta max=\maxfvu,
			nodes near coords dual threshold={0.15 and 0.75},
			height=0.375in,
			ylabel={MLSAE},
			ytick=\empty,
			ymax=+0.5,
		]
		\addplot[
			matrix plot,
			mesh/cols=5,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-70m-deduped-lens-layer/multi_layer/fvu.csv};
		\nextgroupplot[
			point meta min=0,
			point meta max=\maxloss,
			nodes near coords dual threshold={1.5 and 7},
			height=0.375in,
			ymin=1.5,
			ymax=2,
		]
		\addplot[
			matrix plot,
			mesh/cols=5,
			point meta=explicit,
		] table[col sep=comma,meta=value] {test/pythia-70m-deduped-lens-layer/multi_layer/loss.csv};
	\end{groupplot}
\end{tikzpicture}

==> test/pythia-70m-deduped/downstream_loss.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.875in,
			height=1.375in,
			group style={
					group size=2 by 2,
					horizontal sep=0.125in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			cycle list={[colors of colormap={1000,850,...,150}]},
			title style={
					anchor=north,
					at={(0.5,1.1)},
					font=\small
				},
			xmode=log,
			ymode=log,
			grid=major,
			legend cell align={left},
			legend columns=1,
			legend style={
					anchor=west,
					at={(1.05,1)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped/expansion_factor.csv}\ExpansionFactorCSV
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped/sparsity_k.csv}\SparsityKCSV
		\nextgroupplot[
			title={Sparsity $k=32$},
			ylabel={Delta CE loss},
			y label style={anchor=south,at={(-0.2,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=0.001,
			ymax=10,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/layer_5] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=val/loss/delta/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,0.001) -- (axis cs:64,10);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xmin=1e1,
			xmax=1e3,
			ymin=0.001,
			ymax=10,
		]
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/layer_5] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=val/loss/delta/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,0.001) -- (axis cs:32,10);
		\nextgroupplot[
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={KL divergence},
			y label style={anchor=south,at={(-0.2,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=100,
			ymax=12500,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/layer_5] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=val/logit/kldiv/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,100) -- (axis cs:64,12500);
		\nextgroupplot[
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
			ymin=100,
			ymax=12500,
		]
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/layer_5] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=val/logit/kldiv/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,100) -- (axis cs:32,12500);
		\addlegendentry{Layer 0}
		\addlegendentry{Layer 1}
		\addlegendentry{Layer 2}
		\addlegendentry{Layer 3}
		\addlegendentry{Layer 4}
		\addlegendentry{Layer 5 }
		\addlegendentry{Mean}
	\end{groupplot}
\end{tikzpicture}

==> test/pythia-70m-deduped/l1_norm.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.875in,
			height=2.75in,
			group style={
					group size=2 by 1,
					horizontal sep=0.35in,
					x descriptions at=edge bottom,
				},
			cycle list={[colors of colormap={1000,850,...,150}]},
			title style={
					anchor=north,
					at={(0.5,1.075)},
					font=\small
				},
			xmode=log,
			ymode=log,
			grid=major,
			legend cell align={left},
			legend columns=1,
			legend style={
					anchor=west,
					at={(1.05,0.5)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped/expansion_factor.csv}\ExpansionFactorCSV
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped/sparsity_k.csv}\SparsityKCSV
		\nextgroupplot[
			title={Sparsity $k=32$},
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={$L^1$ norm},
			y label style={anchor=south,at={(axis description cs:-0.125,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=55,
			ymax=100,
			ytick={60,70,...,100},
			yticklabels={$60$,$70$,$80$,$90$,$100$},
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/layer_5] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=train/l1/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,55) -- (axis cs:64,100);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
			ymin=40,
			ymax=1500,
		]
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/layer_5] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=train/l1/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,40) -- (axis cs:32,1500);
		\addlegendentry{Layer 0}
		\addlegendentry{Layer 1}
		\addlegendentry{Layer 2}
		\addlegendentry{Layer 3}
		\addlegendentry{Layer 4}
		\addlegendentry{Layer 5 }
		\addlegendentry{Mean}
	\end{groupplot}
\end{tikzpicture}

==> test/pythia-70m-deduped/reconstruction_error.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{groupplot}[
			scale only axis,
			width=1.875in,
			height=1.375in,
			group style={
					group size=2 by 2,
					horizontal sep=0.125in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			cycle list={[colors of colormap={1000,850,...,150}]},
			title style={
					anchor=north,
					at={(0.5,1.1)},
					font=\small
				},
			xmode=log,
			ymode=log,
			grid=major,
			legend cell align={left},
			legend columns=1,
			legend style={
					anchor=west,
					at={(1.05,1)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped/expansion_factor.csv}\ExpansionFactorCSV
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped/sparsity_k.csv}\SparsityKCSV
		\nextgroupplot[
			title={Sparsity $k=32$},
			ylabel={FVU},
			y label style={anchor=south,at={(-0.2,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=0.001,
			ymax=0.4,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/layer_5] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=train/fvu/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,0.001) -- (axis cs:64,0.4);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xmin=1e1,
			xmax=1e3,
			ymin=0.001,
			ymax=0.4,
		]
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/layer_5] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=train/fvu/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,0.001) -- (axis cs:32,0.4);
		\nextgroupplot[
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={MSE},
			y label style={anchor=south,at={(-0.2,.5)}},
			xmin=0.5,
			xmax=512,
			ymin=0.0001,
			ymax=2,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_0] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_1] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_2] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_3] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_4] {\ExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/layer_5] {\ExpansionFactorCSV};
		\addplot+ [dashed,black] table [x=expansion_factor, y=train/mse/avg] {\ExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,0.0001) -- (axis cs:64,2);
		\nextgroupplot[
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
			ymin=0.0001,
			ymax=2,
		]
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_0] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_1] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_2] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_3] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_4] {\SparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/layer_5] {\SparsityKCSV};
		\addplot+ [dashed,black] table [x=k, y=train/mse/avg] {\SparsityKCSV};
		\draw[dashed,gray] (axis cs:32,0.0001) -- (axis cs:32,2);
		\addlegendentry{Layer 0}
		\addlegendentry{Layer 1}
		\addlegendentry{Layer 2}
		\addlegendentry{Layer 3}
		\addlegendentry{Layer 4}
		\addlegendentry{Layer 5 }
		\addlegendentry{Mean}
	\end{groupplot}
\end{tikzpicture}


==> test/with_tuned_lens.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			scale only axis,
			width=2in,
			height=1.25in,
			group style={
					group size=2 by 5,
					horizontal sep=0.375in,
					vertical sep=0.15in,
					x descriptions at=edge bottom,
					ylabels at=edge left,
				},
			cycle list/Paired,
			title style={
					anchor=north,
					at={(0.5,1.1)},
					font=\small
				},
			xmode=log,
			ymode=log,
			grid=major,
			y label style={anchor=south,at={(-0.175,.5)}},
			legend cell align={left},
			legend columns=2,
			legend style={
					anchor=south,
					at={(-0.05,-0.6)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped/expansion_factor.csv}\WithoutTunedLensExpansionFactorCSV
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped/sparsity_k.csv}\WithoutTunedLensSparsityKCSV
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped-lens/expansion_factor.csv}\WithTunedLensExpansionFactorCSV
		\pgfplotstableread[col sep=comma]{test/pythia-70m-deduped-lens/sparsity_k.csv}\WithTunedLensSparsityKCSV
		\nextgroupplot[
			title={Sparsity $k=32$},
			ylabel={FVU},
			xmin=0.5,
			xmax=512,
			ymin=0.005,
			ymax=0.3,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/avg] {\WithoutTunedLensExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/fvu/avg] {\WithTunedLensExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,0.005) -- (axis cs:64,0.3);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xmin=8,
			xmax=1024,
			ymin=0.005,
			ymax=0.3,
		]
		\addplot+ [mark=*] table [x=k, y=train/fvu/avg] {\WithoutTunedLensSparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/fvu/avg] {\WithTunedLensSparsityKCSV};
		\draw[dashed,gray] (axis cs:32,0.005) -- (axis cs:32,0.3);
		\nextgroupplot[
			ylabel={MSE},
			xmin=0.5,
			xmax=512,
			ymin=0.04,
			ymax=2,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/avg] {\WithoutTunedLensExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/mse/avg] {\WithTunedLensExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,0.05) -- (axis cs:64,2);
		\nextgroupplot[
			xmin=8,
			xmax=1024,
			ymin=0.04,
			ymax=2,
		]
		\addplot+ [mark=*] table [x=k, y=train/mse/avg] {\WithoutTunedLensSparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/mse/avg] {\WithTunedLensSparsityKCSV};
		\draw[dashed,gray] (axis cs:32,0.04) -- (axis cs:32,2);
		\nextgroupplot[
			ylabel={$L^1$ norm},
			xmin=0.5,
			xmax=512,
			ymin=60,
			ymax=80,
			ytick={60,70,80},
			yticklabels={$60$,$70$,$80$},
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/avg] {\WithoutTunedLensExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=train/l1/avg] {\WithTunedLensExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,60) -- (axis cs:64,80);
		\nextgroupplot[
			xmin=8,
			xmax=1024,
			ymin=30,
			ymax=1500,
		]
		\addplot+ [mark=*] table [x=k, y=train/l1/avg] {\WithoutTunedLensSparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=train/l1/avg] {\WithTunedLensSparsityKCSV};
		\draw[dashed,gray] (axis cs:32,30) -- (axis cs:32,1500);
		\nextgroupplot[
			ylabel={Delta CE loss},
			ymode=linear,
			xmin=0.5,
			xmax=512,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/avg] {\WithoutTunedLensExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/loss/delta/avg] {\WithTunedLensExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,-10) -- (axis cs:64,10);
		\nextgroupplot[
			ymode=linear,
			xmin=8,
			xmax=1024,
		]
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/avg] {\WithoutTunedLensSparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/loss/delta/avg] {\WithTunedLensSparsityKCSV};
		\draw[dashed,gray] (axis cs:32,-10) -- (axis cs:32,10);
		\nextgroupplot[
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={KL divergence},
			xmin=0.5,
			xmax=512,
			ymin=100,
			ymax=10000,
		]
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/avg] {\WithoutTunedLensExpansionFactorCSV};
		\addplot+ [mark=*] table [x=expansion_factor, y=val/logit/kldiv/avg] {\WithTunedLensExpansionFactorCSV};
		\draw[dashed,gray] (axis cs:64,100) -- (axis cs:64,10000);
		\nextgroupplot[
			xlabel={Sparsity $k$},
			xmin=8,
			xmax=1024,
			ymin=100,
			ymax=10000,
		]
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/avg] {\WithoutTunedLensSparsityKCSV};
		\addplot+ [mark=*] table [x=k, y=val/logit/kldiv/avg] {\WithTunedLensSparsityKCSV};
		\draw[dashed,gray] (axis cs:32,100) -- (axis cs:32,10000);
		\addlegendentry{Pythia-70m}
		\addlegendentry{Pythia-70m with tuned lens}
	\end{groupplot}
\end{tikzpicture}

==> variances/figure.tex <==
\newcommand{\addplotvars}[3]{
	\addplot+ [mark=*] table [
			col sep=comma,
			x=#1,
			y=#2,
		]{#3}
}
\newcommand{\addplotvarsxf}[1]{
	\addplotvars{expansion_factor}{rel_var_f}{#1}
}
\newcommand{\addplotvarsxt}[1]{
	\addplotvars{expansion_factor}{rel_var_t}{#1}
}
\newcommand{\addplotvarskf}[1]{
	\addplotvars{k}{rel_var_f}{#1}
}
\newcommand{\addplotvarskt}[1]{
	\addplotvars{k}{rel_var_t}{#1}
}
\begin{tikzpicture}
	\begin{groupplot}[
			scale only axis,
			width=2in,
			height=2in,
			group style={
					group size=2 by 2,
					horizontal sep=0.125in,
					vertical sep=0.125in,
					x descriptions at=edge bottom,
					y descriptions at=edge left,
				},
			cycle list/Paired,
			title style={
					anchor=north,
					at={(0.5,1.1)},
					font=\small
				},
			y label style={
					anchor=south,
					at={(-0.2,.5)},
					font=\large,
				},
			xmode=log,
			ymode=log,
			grid=major,
			legend cell align={left},
			legend columns=2,
			legend style={
					anchor=south,
					at={(0,-0.75)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\nextgroupplot[
			title={Sparsity $k=32$},
			ylabel={\Large $\frac{\ExpectedValue{\Var(\RandomLayer\mid\RandomLatent)}}{\Var(\RandomLayer)}$},
			xmin=0.5,
			xmax=512,
			ymin=0.15,
			ymax=1,
		]
		\addplotvarsxf{variances/pythia-70m-deduped/expansion_factor.csv};
		\addplotvarsxf{variances/pythia-70m-deduped-lens/expansion_factor.csv};
		\addplotvarsxf{variances/pythia-160m-deduped/expansion_factor.csv};
		\addplotvarsxf{variances/pythia-160m-deduped-lens.csv};
		\addplotvarsxf{variances/pythia-410m-deduped.csv};
		\addplotvarsxf{variances/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotvarsxf{variances/pythia-1b-deduped.csv};
		\addplotvarsxf{variances/pythia-1.4b-deduped.csv};
		\addplotvarsxf{variances/gemma2b.csv};
		\addplotvarsxf{variances/llama3b.csv};
		\addplotvarsxf{variances/gpt2.csv};
		\draw[dashed,gray] (axis cs:64,1e-6) -- (axis cs:64,1);
		\nextgroupplot[
			title={Expansion Factor $\ExpansionFactor=64$},
			xmin=1e1,
			xmax=1e3,
			ymin=0.15,
			ymax=1,
		]
		\addplotvarskf{variances/pythia-70m-deduped/sparsity_k.csv};
		\addplotvarskf{variances/pythia-70m-deduped-lens/sparsity_k.csv};
		\addplotvarskf{variances/pythia-160m-deduped/sparsity_k.csv};
		\addplotvarskf{variances/pythia-160m-deduped-lens.csv};
		\addplotvarskf{variances/pythia-410m-deduped.csv};
		\addplotvarskf{variances/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotvarskf{variances/pythia-1b-deduped.csv};
		\addplotvarskf{variances/pythia-1.4b-deduped.csv};
		\addplotvarskf{variances/gemma2b.csv};
		\addplotvarskf{variances/llama3b.csv};
		\addplotvarskf{variances/gpt2.csv};
		\draw[dashed,gray] (axis cs:32,1e-6) -- (axis cs:32,1);
		\nextgroupplot[
			xlabel={Expansion Factor $\ExpansionFactor$},
			ylabel={\Large $\frac{\ExpectedValue{\Var(\RandomLayer\mid\RandomLatent,\,\RandomToken)}}{\ExpectedValue{\Var(\RandomLayer\mid\RandomLatent)}}$},
			yticklabel style={/pgf/number format/fixed},
			scaled y ticks=false,
			xmin=0.5,
			xmax=512,
			ymin=4e-3,
			ymax=7e-1,
		]
		\addplotvarsxt{variances/pythia-70m-deduped/expansion_factor.csv};
		\addplotvarsxt{variances/pythia-70m-deduped-lens/expansion_factor.csv};
		\addplotvarsxt{variances/pythia-160m-deduped/expansion_factor.csv};
		\addplotvarsxt{variances/pythia-160m-deduped-lens.csv};
		\addplotvarsxt{variances/pythia-410m-deduped.csv};
		\addplotvarsxt{variances/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotvarsxt{variances/pythia-1b-deduped.csv};
		\addplotvarsxt{variances/pythia-1.4b-deduped.csv};
		\addplotvarsxt{variances/gemma2b.csv};
		\addplotvarsxt{variances/llama3b.csv};
		\addplotvarsxt{variances/gpt2.csv};
		\draw[dashed,gray] (axis cs:64,6e-3) -- (axis cs:64,7e-1);
		\nextgroupplot[
			xlabel={Sparsity $k$},
			xmin=1e1,
			xmax=1e3,
			ymin=4e-3,
			ymax=7e-1,
		]
		\addplotvarskt{variances/pythia-70m-deduped/sparsity_k.csv};
		\addplotvarskt{variances/pythia-70m-deduped-lens/sparsity_k.csv};
		\addplotvarskt{variances/pythia-160m-deduped/sparsity_k.csv};
		\addplotvarskt{variances/pythia-160m-deduped-lens.csv};
		\addplotvarskt{variances/pythia-410m-deduped.csv};
		\addplotvarskt{variances/pythia-410m-deduped-lens.csv};
		\pgfplotsset{cycle list/Set2}
		\addplotvarskt{variances/pythia-1b-deduped.csv};
		\addplotvarskt{variances/pythia-1.4b-deduped.csv};
		\addplotvarskt{variances/gemma2b.csv};
		\addplotvarskt{variances/llama3b.csv};
		\addplotvarskt{variances/gpt2.csv};
		\draw[dashed,gray] (axis cs:32,6e-3) -- (axis cs:32,7e-1);
		\addlegendentry{Pythia-70m}
		\addlegendentry{Pythia-70m with tuned lens}
		\addlegendentry{Pythia-160m}
		\addlegendentry{Pythia-160m with tuned lens}
		\addlegendentry{Pythia-410m}
		\addlegendentry{Pythia-410m with tuned lens}
		\addlegendentry{Pythia-1b}
		\addlegendentry{Pythia-1.4b}
		\addlegendentry{Gemma 2 2B}
		\addlegendentry{Llama 3.2 3B}
		\addlegendentry{GPT-2 small}
	\end{groupplot}
\end{tikzpicture}


==> variances/model_name/figure.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
			scale only axis,
			width=4.5in,
			height=1.325in,
			group style={
					group size=1 by 2,
					vertical sep=0.625in,
				},
			xbar,
			y dir=reverse,
			enlarge y limits=true,
			symbolic y coords={
					Pythia-70m,
					Pythia-160m,
					Pythia-410m,
					Pythia-1b,
					Pythia-1.4b,
					gemma-2-2b,
					Llama-3.2-3B,
					gpt2
				},
			ytick=data,
			yticklabels={
					Pythia-70m,
					Pythia-160m,
					Pythia-410m,
					Pythia-1b,
					Pythia-1.4b,
					Gemma 2 2B,
					Llama 3.2 3B,
					GPT-2 small
				},
			xtick align=outside,
			ytick align=outside,
			tick pos=left,
			axis x line*=left,
			axis y line*=left,
			axis line style=semithick,
			every tick/.style={black,semithick},
			legend cell align={left},
			legend columns=1,
			legend style={
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
		]
		\nextgroupplot[
			xlabel={Variance for one latent, aggregating over tokens, as a proportion of the total variance over all latents},
			xmin=0,
			xmax=1,
			bar width=0.0375in,
			legend pos=north east,
		]
		\addplot+ [Paired-A] table [
				col sep=comma,
				y=model_name,
				x=rel_var_f,
			]{variances/model_name/without_tuned_lens.csv};
		\addplot+ [Paired-B] table [
				col sep=comma,
				y=model_name,
				x=rel_var_f,
			]{variances/model_name/with_tuned_lens.csv};
		\addlegendentry{Standard}
		\addlegendentry{Tuned lens}
		\nextgroupplot[
			xlabel={Variance for one token and latent as a proportion of the total variance for that latent},
			xmin=0,
			xmax=0.12,
			bar width=0.0375in,
			scaled x ticks=false,
			xticklabel style={
					/pgf/number format/fixed,
					/pgf/number format/precision=2
				},
			legend pos=north east,
		]
		\addplot+ [Paired-A] table [
				col sep=comma,
				y=model_name,
				x=rel_var_t,
			]{variances/model_name/without_tuned_lens.csv};
		\addplot+ [Paired-B] table [
				col sep=comma,
				y=model_name,
				x=rel_var_t,
			]{variances/model_name/with_tuned_lens.csv};
		\addlegendentry{Standard}
		\addlegendentry{Tuned lens}
	\end{groupplot}
\end{tikzpicture}

==> wdec_sim/figure.tex <==
\begin{tikzpicture}
	\pgfplotsset{
		colormap/viridis high res,
	}
	\begin{groupplot}[
			scale only axis,
			width=2.25in,
			height=1.05in,
			group style={
					group size=2 by 5,
					horizontal sep=0.4in,
					vertical sep=0.35in,
					x descriptions at=edge bottom,
					ylabels at=edge left,
				},
			cycle list/Set1,
			title style={font=\small},
			every axis title/.style={at={(0.5,1.075)}},
			xlabel={Cosine Similarity},
			ylabel={Frequency},
			y label style={anchor=south,at={(-0.15,0.5)}},
			enlarge x limits=0.05,
			grid=major,
			tick pos=left,
			legend cell align={left},
			legend columns=1,
			legend pos=north west,
			legend style={
					anchor=south,
					at={(-0.1,-1)},
					column sep=0.1in,
					draw=none,
					fill=none,
					font=\small,
				},
			unbounded coords=jump,
		]
		%
		\nextgroupplot[
			title={Pythia-70m},
			xmin=-0.2,xmax=+0.2,
			ymin=0,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-70m-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		\nextgroupplot[
			title={Pythia-70m},
			xmin=-1,xmax=+1,
			ymode=log,ymin=1e0,ymax=1e10,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-70m-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		%
		\nextgroupplot[
			title={Pythia-160m},
			xmin=-0.2,xmax=+0.2,
			ymin=0,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-160m-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		\nextgroupplot[
			title={Pythia-160m},
			xmin=-1,xmax=+1,
			ymode=log,ymin=1e0,ymax=1e10,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-160m-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		%
		\nextgroupplot[
			title={Pythia-410m},
			xmin=-0.2,xmax=+0.2,
			ymin=0,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-410m-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		\nextgroupplot[
			title={Pythia-410m},
			xmin=-1,xmax=+1,
			ymode=log,ymin=1e0,ymax=1e10,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-410m-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		%
		\nextgroupplot[
			title={Pythia-1b},
			xmin=-0.2,xmax=+0.2,
			ymin=0,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-1b-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		\nextgroupplot[
			title={Pythia-1b},
			xmin=-1,xmax=+1,
			ymode=log,ymin=1e0,ymax=1e10,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-1b-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		%
		\nextgroupplot[
			title={Pythia-1.4b},
			xmin=-0.2,xmax=+0.2,
			ymin=0,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-1.4b-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		\nextgroupplot[
			title={Pythia-1.4b},
			xmin=-1,xmax=+1,
			ymode=log,ymin=1e0,ymax=1e10,
		]
		\pgfplotstableread[col sep=comma]{wdec_sim/pythia-1.4b-deduped-x64-k32.csv}\Hist
		\addplot+ [const plot mark left] table [x=bins,y=actual] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=positive10] {\Hist};
		\addplot+ [const plot mark left] table [x=bins,y=negative] {\Hist};
		%
		\addlegendentry{{Decoder weight vectors}}
		\addlegendentry{{Paired normal i.i.d. vectors plus noise (positive control)}}
		\addlegendentry{{Normal i.i.d. vectors (negative control)}}
	\end{groupplot}
\end{tikzpicture}
